Self-Supervised Representation Learning from Temporal Ordering of Automated Driving Sequences

Self-supervised feature learning enables perception systems to benefit from the vast raw data recorded by vehicle fleets worldwide. While video-level self-supervised learning approaches have shown strong generalizability on classification tasks, the potential to learn dense representations from sequential data has been relatively unexplored. In this work, we propose TempO, a temporal ordering pretext task for pre-training region-level feature representations for perception tasks. We embed each frame by an unordered set of proposal feature vectors, a representation that is natural for object detection or tracking systems, and formulate the sequential ordering by predicting frame transition probabilities in a transformer-based multi-frame architecture whose complexity scales less than quadratic with respect to the sequence length. Extensive evaluations on the BDD100K, nuImages, and MOT17 datasets show that our TempO pre-training approach outperforms single-frame self-supervised learning methods as well as supervised transfer learning initialization strategies, achieving an improvement of +0.7% in mAP for object detection and +2.0% in the HOTA score for multi-object tracking.

==> sections/31_loss_pseudo_code.tex <==
\begin{algorithm}
\small
\SetAlgoLined
\KwData{Image sequence $\mathcal{I}_1, \dots  \mathcal{I}_N$ in correct temporal order, margin $m$}
\KwResult{$\mathcal{L}_{TempO}$}
    \ForAll {$\mathcal{I}_i$}{
        $\mathcal{T}_i = \textit{SpatialNetwork}\left(\mathcal{I}_i \right)$ 
    }
    {\color{cyan}\# per-frame track tokens $\mathbf{T}_{i} \in \mathbf{R}^{Q \times D}$ \;}
    $\mathbf{H}_{1:N-1} = \textit{HistoryEncoder} \left(  [\mathcal{T}_1, \dots, \mathcal{T}_{N-1}], \mathcal{M}_{\textit{future}} \right)$ \;
    {\color{cyan}\# history tokens $\mathbf{H}_{1:N-1} \in \mathbf{R}^{(N-1) \cdot Q \times D}$ \;}
    % \For{$i \in [1, \dots, N-1]$}{
    %     $\mathbf{S} = \textit{AdditiveAttention}(\mathbf{Q}_{i}, \mathbf{T}_{i+1:N} )$ \;
    % }
    % {\color{cyan}\# matching scores $\mathbf{S}_{i} \in \mathbf{R}^{(N-i-1) \times P \times P}$ \;}
    % {\color{cyan}\# slice $\mathbf{S}^{i}$ into matching scores by frame-pair \;}
    
    

    % $\mathcal{L}_{TempO}$ = 0 \;
    % \For{$i \in [1, \dots, N-1]$}{
    %     {\color{cyan}\# for temporally consecutive frame pair (positives), compute row-wise maximum association score\;}
    %     $p_{i,i+1}$ = $[ \max\left\{\mathbf{s}^{i,i+1}_1\right\}, \max\left\{\mathbf{s}^{i,i+1}_2\right\}, \dots, \max\left\{\mathbf{s}^{i,i+1}_P\right\} ]$\;
    %     \For{$j \in [i+2, \dots, N]$}{
    %         {\color{cyan}\# for temporally non-consecutive frame pair (negatives), compute row-wise maximum association score\;}
    %         $n_{i,j}$  = $[ \max\left\{\mathbf{s}^{i,j}_1\right\}, \max\left\{\mathbf{s}^{i,j}_2\right\}, \dots, \max\left\{\mathbf{s}^{i,j}_P\right\} ]$ \;
    %         $\mathcal{L}_{TempO}$ += $\max\left\{ n_{i,j} - p_{i,i+1} + m ,0 \right\}$ 
    %     }
    % }
    
    
    
    $\mathcal{L}_{TempO}$ = 0 \;
    \For{$i \in [2, \dots, N]$}{
        {\color{cyan}\# matching scores $\mathbf{S}_{i} \in \mathbf{R}^{(N-i-1) \times P \times P}$ \;}
        $\mathbf{S}_{i,i-1} = \textit{AdditiveAttention}(\mathbf{T}_{i}, \mathbf{H}_{i-1} )$ \;
        $p_{i,i-1} = \textit{ReductionFunction}(\mathbf{S}_{i,i-1})$\;
        \For{$j \in [1, \dots, N-1] \And j \neq i-1 $}{
            $\mathbf{S}_{i,j} = \textit{AdditiveAttention}(\mathbf{T}_{i}, \mathbf{H}_{j} )$ \;
            $n_{i,j} = \textit{ReductionFunction}(\mathbf{S}_{i,j})$\;
            $\mathcal{L}_{TempO}$ += $\max\left\{ n_{i,j} - p_{i,i-1} + m ,0 \right\}$ 
        }
    }
    
\caption{TempO pretext task pipeline.}
\label{fig:pseudo_code}
\end{algorithm}

==> sections/46_reduction_function.tex <==
Since tracking requires a consistent embedding of an object across subsequent frames, we also experiment to enforce a one-to-one matching among track features of two frames as a reduction function from a set of per-frame proposal feature vectors to scalar image transition probabilities. 
Therefore, we propose an approximation of the linear sum assignment as follows:
\begin{align}
    \rho \left( \mathbf{T}_n | \mathbf{H}_{m} \right) =  \sum_j \max_j \left[ \underset{i=1,\dots,P}{\text{softmax}} \left( Att( \mathbf{t}_n^i, \mathbf{h}_{m}^j ) \right) \right]
    \label{eq:reduction_function_max}
\end{align}
and ablate over these choices of the reduction function. The comparison the AvgPool reduction is shown in \figref{tab:supp_ablation}. From these results, we find that using \eqref{eq:reduction_function_max} as a reduction function for the association score matrices resulted in a drop in performance compared to average pooling by $-0.7\%mAP$, which we assume to be a result of the sparser and attenuated gradients.

\begin{table*}
\footnotesize
\centering
\caption{Ablation experiments on downstream tasks for various TempO pre-training settings. All experiments use a Sparse R-CNN object detector with a ResNet-50 backbone and 100 proposals per frame.}
\label{tab:supp_ablation}
\begin{tabular}{cccc|llllll|llll}
\toprule
\multicolumn{4}{c}{Pretext setting} & \multicolumn{6}{c}{BDD100k val object detection} & \multicolumn{4}{c}{BDD100k val MOT} \\
$N_{seq}$ & $L_{\{enc, dec\}}$ & $f_{sim}$ & Augment. & AP & AP50 & AP75 & APs & APm & APl & HOTA ↑ & sMOTA ↑ & IDF1 ↑ & IDSw. ↓ \\ \midrule
8 & 2 & AvgPool & -  & \textbf{31.4} & \textbf{57.3} & \textbf{29.5} & \textbf{15.7} & \textbf{35.2} & \textbf{51.6} & 
36.6 & 26.3 & 40.5 & 90388\\
8 & 2 & MSA & -  & 30.7 & 55.9 & 29.0 & 15.1 & 34.4 & 25.1 & 
35.3 & 25.9 & 40.4 & 91600 \\ 
\bottomrule
\end{tabular}
\end{table*}

==> tables/ablation_det_convergence_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\scriptsize
\centering
\caption{V2 Object detection results on BDD100k val dataset for increasing number of fine-tuning epochs. The TempO pre-training used a sequence length of 8 frames, two layers in the multi-frame network, as well as AvgPool motivated by \tabref{tab:ablation}. }
\label{tab:ablation_det_convergence}
\begin{tabular}{lll|p{0.35cm}p{0.35cm}p{0.35cm}p{0.35cm}p{0.35cm}p{0.35cm}} \toprule
Model & Pre-train & Epoch &  \multicolumn{6}{c}{BDD100k val object detection} \\
& & & AP & AP50 & AP75 & APs & APm & APl \\ \midrule
\multirow{8}{*}{SparseRCNN} & COCO & 2 & 21.1 & 37.6 & 20.2 & 8.8 & 23.9 & 40.5 \\
 & TempO & 2 & 20.7 & 40.4 & 18.4 & 9.6 & 23.8 & 36.5 \\
 & COCO & 4 & 22.7 & 40.6 & 21.7 & 10.1 & 26.0 & 41.1 \\
 & TempO & 4 & 26.5 & 49.7 & 24.2 & 13.1 & 30.1 & 43.3 \\ 
 & COCO & 6 & 25.1 & 43.8 & 24.4 & 10.8 & 28.6 & 46.3 \\
  & TempO & 6 & 30.7 & 55.8 & 28.9 & 15.2 & 34.3 & 50.7 \\ 
 & COCO & 12 & 30.7 & 55.8 & 28.9 & 15.2 & 34.3 & 50.8 \\ 
 & TempO & 12 & 31.3 & 57.1 & 29.2 & 15.2 & 35.1 & 52.3 \\ \midrule
 \multirow{8}{*}{DDETR} & COCO & 2 & 9.3 & 20.9 & 6.9 & 4.5 & 11.6 & 17.3 \\
  & TempO & 2 & 13.9 & 29.9 & 11.3 & 6.1 & 16.6 & 26.6 \\
 & COCO & 4 & 16.8 & 34.7 & 14 & 7.6 & 19.8 & 30.6 \\
 & TempO & 4 & 30.6 & 55.9 & 28.3 & 12.7 & 34.3 & 55.0 \\ 
 & COCO & 6 & 28.3 & 52.2 & 26.1 & 11.2 & 32.1 & 53.6 \\
 & TempO & 6 & 31.3 & 57.9 & 28.9 & 15.2 & 34.9 & 55.3 \\ 
 & COCO & 12 & 30.2 & 56.0 & 27.6 & 14.2 & 34.0 & 51.3 \\ 
 & TempO & 12 & \textbf{32.5} & \textbf{59.2} & \textbf{30.4} & \textbf{15.7} & \textbf{36.9} & \textbf{55.3} \\ \bottomrule
\end{tabular}
\end{table}



==> tables/eval_semseg_bdd100k.tex <==
\begin{table}[ht]
\scriptsize
\centering
\caption{Semantic Segmenation performance evaluation on BDD100k test set.}
\label{tab:eval_semseg_bdd100k_test}
\begin{tabular}{llllllcccccccc}
\toprule
Model & Architecture &  &  & Initialization & \multicolumn{8}{c}{BDD100k test} \\
 & BackBone & Head & Patch size &  & mIoU & ACC & fIoU & pAcc & mIoU & ACC & fIoU & pAcc \\ \midrule
ViT-B \cite{dosovitskiy2020image} & ViT-B & UPerHead & 16 & ImageNet & 62.1 & 79.1 & 88.5 & 93.7 & 54.0 & 76.0 & 86.0 & 92.2 \\
DPT \cite{ranftl2021vision} & ViT-B & DPTHead & 16 & ImageNet & 63.5 & 79.1 & 89.2 & 94.1 & 54.7 & 79.9 & 86.3 & 92.4 \\
DeiT & DeiT-S & UPerHead & 16 & DeiT & 61.5 & 77.7 & 88.3 & 93.6 & 53.4 & 77.2 & 85.7 & 92.0 \\
 &  &  &  &  &  &  &  &  &  &  &  & \\ \bottomrule
\end{tabular}
\end{table}

==> tables/rebutall_training_times.tex <==
\begin{table}[h]
\centering
\scriptsize
\caption{Pre-training runtimes for TempO approach using a batch size of 8 and 4 Nvidia V100 GPUs.}
\label{tab:training_runtimes}
\begin{tabular}{lllllll} \toprule
$N_{seq}$ & $L_{enc,dec}$ & \# data points & Num epochs & Datasamples/s & GPUh  & GPU days \\ \midrule
8       & 4     & 2M            & 6          & 7.9           & 420.8 & 17.5     \\
8       & 2     & 2M            & 6          & 8.2           & 406.5 & 16.9     \\
8       & 1     & 2M            & 6          & 8.7           & 383.3 & 16.0     \\
6       & 2     & 2.64M         & 6          & 9.2           & 478.5 & 19.9     \\
4       & 2     & 4M            & 6          & 12.1          & 550.0 & 22.9    \\ \bottomrule
\end{tabular}
\end{table}

==> tables/rebuttal.tex <==
\begin{table}[h]
\scriptsize
\centering
\caption{Comparison of selected datasets by the requirements for TempO evaluation.}
\label{tab:dataset-comparison}
\begin{tabular}{llllllll} \toprule
Dataset name     & Total images & Object detection split & Object categories & Total sequence length [h] & 2D Det & 2D MOT & Unannotated set                 \\ \midrule
BDD100k~\cite{yu2020bdd100k}          & 20M          & 70k/10k/20k            & 10                & 1000                 & \checkmark          & \checkmark         & 80k - 1000k videos a 40s \\
nuScenes~\cite{caesar2020nuscenes}         & 1.4M         & 60k/16k/16k              & 10                & 5.5                  & \checkmark           & -          & sweep recordings        \\
KITTI 360~\cite{liao2022kitti}       & 15k          & 7k/8k/-                & 8                 & 1.5                 & \checkmark          & \checkmark         &                                 \\
COCO 2017~\cite{lin2014microsoft}       & 330k         & 118K/5K/41K            & 80                & -                     & \checkmark          & -          & 123k images                     \\
Open Images V7~\cite{kuznetsova2020openimages}   &              & 1.7M/41k/125k          & 600               & -                     & \checkmark          & -          & 9M - 1,9M images                \\
YouTube VIS 2021~\cite{xu2018youtubevos} &              & 3k/421/453             & 40                & 5.6                  & \checkmark          & -          &                     \\ \bottomrule          
\end{tabular}
\end{table}

==> utils/equation_dump.tex <==
\begin{align}
     \rho\left( \mathbf{t_i} \mid \mathbf{I}  \right) = 
         \underbrace{\rho\left( \mathbf{t_i} \mid pg  \right)}_\text{task-specific score} \cdot 
         \underbrace{\rho\left( pg \mid \mathbf{\Theta},  \mathbf{\Delta}  \right)}_\text{bottom-up generation} \cdot 
         \underbrace{\rho\left( \mathbf{\Theta} \mid \mathbf{I} \right)}_\text{token extraction}
\end{align}

\begin{align}
 \rho\left( \mathbf{t_i} \mid \mathbf{I}  \right) = 
 \underbrace{\rho\left( \mathbf{t_i} \mid pg  \right)}_\text{task-specific score} \cdot 
 \underbrace{\rho\left( pg \mid \mathbf{\Theta},  \mathbf{\Delta}  \right)}_\text{parse-graph generation} \cdot 
 \underbrace{\rho\left( \mathbf{\Theta} \mid \mathbf{I} \right)}_\text{token extraction}
\end{align}

\begin{align}
    \arg \underset{pg}{ \max } \rho (\mathbf{I} \mid pg) \cdot \rho (pg \mid \mathbf{\Theta}, \mathbf{\Delta})
\end{align}

\begin{align}
     \rho\left( pg \mid \mathbf{\Theta},  \mathbf{\Delta}  \right) = 
 \prod_{l \in [1, \dots, L-1]} \left(
    \underbrace{
    \prod_{\mathbf{c}^{l-1}_j \in \mathbf{C}^{l-1}} 
        \max_{\mathbf{c}^l_k \in \mathbf{C}^l} \rho( \mathbf{c}^l_k \mid \mathbf{c}^{l-1}_j )
        }_{\rho (\mathbf{C}^l \mid \mathbf{C}^{l-1})}
 \right) \cdot
    \underbrace{
    \prod_{\mathbf{\theta} \in \mathbf{\Theta}} \left( \max_{c^0_i \in \mathbf{C}^0} \rho(c^0_i \mid \theta) \cdot \rho (\theta) \right)}_{\rho(\mathbf{C}^0 \mid \mathbf{\Theta})}
\end{align}

\begin{align}
         \rho\left( pg \mid \mathbf{\Theta},  \mathbf{\Delta}  \right) = 
 \prod_{l \in [L-1, \dots, 1]} \left(
    \prod_{\mathbf{c}^{l}_j \in \mathbf{C}^{l}} 
        \max_{\mathbf{c}^{l-1}_k \in \mathbf{C}^{l-1}} \rho( \mathbf{c}^{l-1}_k \mid \mathbf{c}^{l}_j )
 \right) \cdot
    \prod_{\mathbf{\theta} \in \mathbf{\Theta}} \left( \max_{c^0_i \in \mathbf{C}^0} \rho(c^0_i \mid \theta, \mathbf{C}_0) \cdot \rho (\theta) \right)
\end{align}

\begin{align}
    Att(Q, K, V) = Corr(Q, K) V = softmax \left( \frac{Q K^T}{\sqrt{C}} \right) V
\end{align}



\begin{align}
    CrossAtt_l = arg \max_{l} \text{ softmax}\left( (\mathbf{W}_K \mathbf{C}^l) (\mathbf{W}_Q \mathbf{C}^{l-1} )^T \right)
\end{align}

\begin{align}
    arg \max_{\mathbf{S}} \rho \left( \mathbf{S}^* \right) % I_{t+1} = b_j \mid I_{t} = b_i \right), \forall j \neq i
\end{align}

\begin{align}
    arg \max_{\mathbf{S}} \prod^{N-1}_{n=1} \rho \left( s_n \mid \mathbf{S}_{0:n} \right)
\end{align}

